Learning Markerless Robot-Depth Camera Calibration and End-Effector Pose Estimation

Traditional approaches to extrinsic calibration use fiducial markers and learning-based approaches rely heavily on simulation data. In this work, we present a learning-based markerless extrinsic calibration system that uses a depth camera and does not rely on simulation data. We learn models for end-effector (EE) segmentation, single-frame rotation prediction and keypoint detection, from automatically generated real-world data. We use a transformation trick to get EE pose estimates from rotation predictions and a matching algorithm to get EE pose estimates from keypoint predictions. We further utilize the iterative closest point algorithm, multiple-frames, filtering and outlier detection to increase calibration robustness. Our evaluations with training data from multiple camera poses and test data from previously unseen poses give sub-centimeter and sub-deciradian average calibration and pose estimation errors. We also show that a carefully selected single training pose gives comparable results.

==> algo.tex <==

% \begin{minipage}{0.46\textwidth}
% \begin{algorithm}[H]
%     \centering
%     \caption{Outlier Detection}\label{algorithm}
%     \begin{algorithmic}[1]
%         \State \text{findOutliers (lst)} 
%         \State $\textit{m} \gets \text{2.0}$
%         \State $d \gets \lvert \text{lst} - \text{med(lst)}\rvert $
%         \State $mdev \gets \text{med(d)} $
        
%         \If{$mdev \neq 0$}
%             \State $s \gets d/mdev $\;
%         \Else 
%             \State $s \gets \text{0} $\;
%         \EndIf 
        
%         \State \textbf{Return}  s \textgreater` m
%     \end{algorithmic}
% \end{algorithm}
% \end{minipage}
% \hfill
% \begin{minipage}{0.46\textwidth}
% \begin{algorithm}[H]
%     \centering
%     \caption{Find}\label{algorithm1}
%     \begin{algorithmic}[1]
%         \State \text{dataProcessing (dataset)} 
%         \State $\textit{unitToDrop} \gets \text{25\%}$
%         \State \text{text}
%         \State \text{text}
%         \Repeat
%         \State \text{/*text*/}
%         \For{$i\gets 1, rows$}
%         \State $\text{text}$ 
%         \State $\text{text}$ 
%         \State $\text{text}$ 
%         \State \text{text}
%         \State $\text{text}$
%         \EndFor
%         \Until {text}
%         \State \text{text}
%         \Repeat
%         \State \text{text}
%         \For{$i\gets 1, rows$}
%         \State $\text{text}$ 
%         \State $\text{v}$ 
%         \EndFor
%         \Until {text}
%         \State \textbf{Return}  \text{text, text}
%     \end{algorithmic}
% \end{algorithm}
% \end{minipage}
